Data-driven Estimation of Origin-Destination Demand and User Cost Functions for the Optimization of Transportation Networks

In earlier work (Zhang et al., 2016) we used actual traffic data from the Eastern Massachusetts transportation network in the form of spatial average speeds and road segment flow capacities in order to estimate Origin-Destination (OD) flow demand matrices for the network. Based on a Traffic Assignment Problem (TAP) formulation (termed "forward problem"), in this paper we use a scheme similar to our earlier work to estimate initial OD demand matrices and then propose a new inverse problem formulation in order to estimate user cost functions. This new formulation allows us to efficiently overcome numerical difficulties that limited our prior work to relatively small subnetworks and, assuming the travel latency cost functions are available, to adjust the values of the OD demands accordingly so that the flow observations are as close as possible to the solutions of the forward problem. We also derive sensitivity analysis results for the total user latency cost with respect to important parameters such as road capacities and minimum travel times. Finally, using the same actual traffic data from the Eastern Massachusetts transportation network, we quantify the Price of Anarchy (POA) for a much larger network than that in Zhang et al. (2016).

==> mymacros.tex <==
% Equations ... 
\newcommand{\be}[1]{\begin{equation}\label{#1}}
\newcommand{\benon}{\begin{equation*}}  
%\newcommand{\ee}{\end{equation}}
%\newcommand{\eenon}{\end{equation*}}
\newcommand{\bemuln}[1]{\begin{multline}\label{#1}}
\newcommand{\bemul}{\begin{multline*}}
%\newcommand{\emuln}{\end{multline}}
%\newcommand{\emul}{\end{multline*}}
\newcommand{\bee}{\begin{eqnarray*}}
\newcommand{\eee}{\end{eqnarray*}}
\newcommand{\been}[1]{\begin{eqnarray}\label{#1}}
\newcommand{\eeen}{\end{eqnarray}}
\newcommand{\began}[1]{\begin{gather}\label{#1}}
\newcommand{\bega}{\begin{gather*}}
%\newcommand{\egan}{\end{gather}}
%\newcommand{\ega}{\end{gather*}}
\newcommand{\bealn}[1]{\begin{align}\label{#1}}
\newcommand{\beal}{\begin{align*}}
%\newcommand{\ealn}{\end{align}}
%\newcommand{\eal}{\end{align*}}
\newcommand{\bealatn}[2]{\begin{alignat}{#1}\label{#2}}
\newcommand{\bealat}{\begin{alignat*}}
%\newcommand{\ealatn}{\end{alignat}}
%\newcommand{\ealat}{\end{alignat*}}
\newcommand{\bexalatn}[1]{\begin{xalignat}\label{#1}}
\newcommand{\bexalat}{\begin{xalignat*}}
%\newcommand{\exalatn}{\end{xalignat}}
%\newcommand{\exalat}{\end{xalignat*}}


% Various...
\newcommand{\qed}{\newline \mbox{ } \hfill 
             \rule[-1pt]{2.5mm}{2.5mm}\par\vskip 10pt }
\newcommand{\inlineqed}{\hfill 
             \rule[-1pt]{2.5mm}{2.5mm}\par\vskip 10pt }
\newcommand{\ra}{\rightarrow}
\newcommand{\Ra}{\Rightarrow}
\newcommand{\pf}{\vskip 5 pt \noindent {\bf{Proof : }}}
\newcommand{\disc}{\vskip 5 pt \noindent {\bf Discussion : }}
\newcommand{\mot}{\vskip 5 pt \noindent {\bf Motivation : }}
%\newcommand{\note}{\vskip 5 pt \noindent {\bf Note : }}
\newcommand{\rems}{\vskip 5 pt \noindent {\bf Remarks : }}
\newcommand{\rem}{\vskip 5 pt \noindent {\bf Remark : }}
%\newcommand{\Nt}{{\tilde N}}
\newcommand{\diag}{\text{diag}}

%Font commands
\newcommand{\mb}{\mathbf}
\newcommand{\bsy}{\boldsymbol}
\newcommand{\mn}{\mathnormal}
\newcommand{\mbb}{\mathbb}
\newcommand{\bosy}{\boldsymbol}


% Theorems ...
{\theoremstyle{plain} \newtheorem{thm}{Theorem}[section]
\newtheorem{conj}[thm]{Conjecture}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{lemma}[thm]{Lemma}
\newtheorem{algo}[thm]{Algorithm}
\newtheorem{cor}[thm]{Corollary}}
{\theoremstyle{break} \theorembodyfont{\it}
\newtheorem{defi}{Definition}
\newtheorem{ass}{Assumption} 
\newtheorem{cond}{Condition}}
\renewcommand{\theass}{\Alph{ass}} 

%Style
%\newlength{\captionwidth}
%\setlength{\captionwidth}{\textwidth}
%\addtolength{\captionwidth}{-1in}
%\newsavebox{\mytempbox}
%\makeatletter
%\renewcommand{\@makecaption}[2]{%redefine makecaption length=\captionwidth
%	\par\vspace{10pt}
%	\sbox{\mytempbox}{{\bf #1}: {\small #2}}%
%	\ifdim \wd\mytempbox > \linewidth
%	{\begin{center}\parbox[t]{\captionwidth}{{\bf #1}: {\small #2}}
%		\end{center}}
%	\else
%	{\begin{center}{\bf #1}: {\small #2}\end{center}}
%	\fi
% }
%\renewcommand{\@makecaption}[2]{%redefine makecaption lenght=\textwidth
%	\vspace{10pt}
%	\sbox{\mytempbox}{{\bf #1}: {\small #2}}%
%	\ifdim \wd\mytempbox > \linewidth
%	{{\bf #1}: {\small #2}\par}% more than one line
%	\else
%	{\begin{center}{\bf #1}: {\small #2}\end{center}}
%	\fi
% }
\makeatother



